A Comparison of Limit Setting Methods for the On-Off Problem

We study the frequentist properties of confidence intervals for the On-Off problem. The methods include all those in common use today. We derive explicit formulas for the limits and calculate the true coverage and the expected lengths of these methods.

==> tbl5-90.tex <==
\begin{table}[tbh]
\caption{Worst coverage of each method, for $0.5\leq b\leq 10$ and $0\leq 
        \protect\mu \leq 20$. $\protect\tau =$ 5 $ and $ 90 $\%$ confidence intervals}
\label{tab:worst5.90}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
&    RLC   &     FCD2   &   FCPL &   FCCH1   &   FCCH2   &    NeyProb   &     CLs  \\
\hline
\hline
b  & $  $  \\
\hline
$\protect\mu $  & $  $  \\
\hline
Coverage    & $  $  \\
\hline
\end{tabular}
\begin{tabular}{|c|c|c|c|c||c|}
\hline
&  $1$ &  $1/\sqrt{\mu }$ & $1/\sqrt{b}$ & $1/\sqrt{\mu b }$ & $1/\sqrt{\mu +b}$ \\
\hline
\hline
b  & $  $  \\
\hline
$\protect\mu $  & $  $  \\
\hline
Coverage    & $  $  \\
\hline
\end{tabular}
\end{table}

